A Micro-Ellipsoid Model for Wet Porous Materials Rendering

Wet porous materials, like wet ground, moist walls, or wet cloth, are common in the real world. These materials consist of transmittable particles surrounded by liquid, where the individual particle is invisible in the macroscopic view. While modeling wet porous materials is critical for various applications, a physically based model for wet porous materials is still absent. In this paper, we model these appearances in the media domain by extending the anisotropic radiative transfer equation to model porosity and saturation. Then, we introduce a novel particle model -- micro-ellipsoid -- by treating each particle as a transmittable ellipsoid, analogous to a micro-flake, to statistically characterize the overall optical behavior of the medium. This way, the foundational theory for media with porosity and saturation is established. Building upon this new medium, we further propose a practical bidirectional scattering distribution function (BSDF) model within the position-free framework--WetSpongeCake. As a result, our WetSpongeCake model is able to represent various appearances of wet porous materials using physical parameters (e.g., porosity and saturation), allowing both reflection and transmission. We validated our model through several examples: a piece of wet cloth, sand saturated with different liquids, or damp sculptures, demonstrating its ability to match real-world appearances closely.

==> 3-sec_background.tex <==
\section{Background and overview}


\subsection{SpongeCake}

\added{}

\subsection{Hapke's model}
\added{
原始辐射传输方程
(In this equation all quantities depend on position, so this dependence is left implicit for
compactness.)
}
\begin{equation}
    \begin{aligned}
(\omega \cdot \nabla) L(\omega)=-\sigma_{t} L(\omega)+\sigma_{s} \int_{\Omega} f_{p}\left(\omega^{\prime} \cdot \omega\right) L\left(\omega^{\prime}\right) \mathrm{d} \omega^{\prime}
\end{aligned}
\end{equation}

\added{
然后得出传统Transmittance
}
\begin{equation}
    \begin{aligned}
T(t) = e^{-\sigma_t t}
\end{aligned}
\end{equation}

\added{
被Hapke改成了$T_H$，其中$K$是和$\sigma_t$与$l$有关的中间量，$l$是粒子间平均距离，被单位内平均粒子数$n$定义。
}
\begin{equation}
    \begin{aligned}
T_H(t)& = Ke^{-K\sigma_t t}\\
K&=-\frac{\ln{(1-\sigma_tl)} }{\sigma_t l} \\
l&=n^{-\frac{1}{3} } \\
\end{aligned}
\end{equation}




==> pseudocode.tex <==
% \newcommand{\mycommfont}[1]{\small\texttt{\textcolor[HTML]{4D8F33}{#1}}}
% \SetCommentSty{mycommfont}

% We show pseudo-code of segment term evaluation in Algorithm \ref{alg:SegmentTerm}, BRDF evaluation in Algorithm \ref{alg:eval} and sample in Algorithm \ref{alg:sample}.

% \newpage

% \begin{algorithm}
% \caption{SegmentTerm}
% \label{alg:SegmentTerm}
% \Class(\tcp*[h]{Initialize $\Lambda_o$}){$\mathrm{SegmentTerm}(\Lambda_o)$} {

%     \Def{$m \gets 1$} \;
%     \Def{$N \gets 0$} \;
%     \Def{$e[], g[], l[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%        \eIf(\tcp*[h]{Downwards}){$\Lambda_k < 0$} {
%         $N \gets N+1$\;
%         $l[N] \gets |\Lambda_k|$\;
%         $e[N] \gets \frac{1}{\Lambda_o+|\Lambda_k|}$\;
%         $g[N] \gets 0$\;
%         $m \gets m \cdot e[N]$\Comment{cache the results when sampled rays are only downwards}
%         }(\tcp*[h]{Upwards}){
        
%             \eIf{$m = 0$}{
%                $g[N] \gets \frac{g[N]}{\Lambda_k + l[N]}$\;
%         }(\tcp*[h]{Initialize g}){
%                $g[N] \gets \frac{1}{\Lambda_k + l[N]}$\;
%                $m \gets 0$\;
%             }

%             \For{$i \gets N-1 ... 1$}{
%                 $g[i] \gets \frac{g[i] + g[i + 1]}{\Lambda_k + l[i]}$\;
%             }
%         }
%     }

%     \Fn{$\mathrm{getS_k}()$}{

%         \If(\tcp*[h]{Return results if cached}){$m \ne 0$}{
%         \KwRet{ m }\;
%         }
%          $s \gets 0$\;
%         \For{$i \gets N ... 1$}{
%             $s \gets e[i] \cdot (s + g[i])$\;
%         }
%         \KwRet{ s }\;
    
%     }
% }

% \end{algorithm}


% \begin{algorithm}
% \caption{Eval}
% \label{alg:eval}
% \Fn{$\mathrm{eval}(\omega_i,\omega_o)$}{
% $\mathrm{SegmentTerm} \  s(\Lambda(\omega_o))$\Comment{ initializing }
% $f \gets 0$\Comment{result}
% $k \gets 0$ \Comment{bounce}
% $w \gets 1$\Comment{weight}
% $\bd_0 \gets -\omega_i$\;
% \While{$\mathrm{true}$}{
%     $s.\mathrm{addBounce}(\Lambda(\bd_{k}))$\;
%     $k \gets k + 1$\;
%     \If{$k >= rrDepth$}{
%         \If{$\mathrm{rand}()>q$}{
%         break;
%         }
%     $w \gets {w \over q}$\Comment{russian roulette}
%     }
%     $f \gets f + w \cdot v(\bd_{k},\omega_o)\cdot s.\mathrm{getS_k}() $\;
%     \If{$k \ge maxBounce$}{
%         break;
%     }
%     ($\bd_{k+1}$,$p_k$) $ \gets $ sample($ \bd_{k} $)\;
%     $w \gets {w \cdot v(\bd_{k},\bd_{k+1}) \over p_k}$\;
% }
%         \KwRet{ f }\;
% }
% \end{algorithm}

% \begin{algorithm}
% \caption{Sample}
% \label{alg:sample}
% \KwResult{weight $w$ and direction $\bd_k$}
% \BlankLine
% $p \gets 1$  \Comment{pdf}
% $k \gets 0$  \Comment{bounce}
% $w \gets 1$  \Comment{weight}
% $\bd_0 \gets -\omega_i$\;
% \While{$\mathrm{true}$}{
%    ($\bd_k$,$p_k$,$w_k$) $ \gets $ sample($ \bd_{k-1} $)\;
%    $w \gets w \cdot w_k$\;
%    $p \gets p \cdot p_k$\;
%     \If{$\bd_k.z > 0$}{
%     $G_1 \gets \frac{1}{|\Lambda(\bd_k)|}$\;
%         \eIf(\tcp*[h]{the ray continues the tracing with $G_1$ as the probablity}){$\mathrm{rand()}<G_1$}
%         {
%             $p \gets p \cdot G_1$\;
%             break;
%         }{
%             $p \gets p \cdot (1-G_1)$\;
%         }
%     }
% $k \gets k+1$\;
%     \If{$k \ge maxBounce$}{
%         break;
%     }
% }
%    $w \gets w \cdot S_k(\bd_0,...,\bd_k)$\;
%    $w \gets {w \over p}$\;
% \end{algorithm}

% \newcommand{\mybox}[3]{
% \begin{tcolorbox}[arc = 0pt, outer arc = 0pt,
%     colback = #1!10!white, colframe = #1!70!black,
%     boxsep = 0pt, left = 2pt, right = 2pt, top = 2pt, bottom = 2pt,
%     boxrule = 0pt, bottomrule = 1pt, toprule = 1pt,width=#2]
% #3
% \end{tcolorbox}
% }

% \newpage

% \begin{algorithm}[h]
% \caption{SegmentTerm}
% \label{alg:coloredST}
% \Class{$\mathrm{SegmentTerm}(\Lambda_o)$} {

%     $N \gets 0$ \;
%     $m \gets 1$ \;
%     \Def{$e[], g[], l[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%        \eIf{$\Lambda_k < 0$} {
%       \mybox{green}{24mm}{
%        % \begin{mybox}[width=30mm]
%        $N \gets N+1$\;
%         % \end{mybox}
%         $l[N] \gets |\Lambda_k|$\;
%         $e[N] \gets \frac{1}{\Lambda_o+|\Lambda_k|}$\;
%         $g[N] \gets 0$\;
%         $m \gets m \cdot e[N]$\;
%         }
%         }{
        
%     \mybox{yellow}{33.5mm}{
%             \eIf{$m = 0$}
%             {
%                $g[N] \gets \frac{g[N]}{\Lambda_k + l[N]}$\;
%         }{
%                $g[N] \gets \frac{1}{\Lambda_k + l[N]}$\;
%                $m \gets 0$\;
%             }
% \mybox{red}{32mm}{
%             \For{$i \gets N-1 ... 1$}{
%                 $g[i] \gets \frac{g[i] + g[i + 1]}{\Lambda_k + l[i]}$\;
%             }}
%             }
%         }
%     }

%     \Fn{$\mathrm{getS_k}()$}{
%     \mybox{cyan}{33.5mm}{
%         \If{$m \ne 0$}{
%         \KwRet{ m }\;
%         }
%          $s \gets 0$\;
         
% \mybox{red}{32mm}{
%         \For{$i \gets N ... 1$}{
%             $s \gets e[i] \cdot (s + g[i])$\;
%         }}
%         \KwRet{ s }\;
%     }
%     }
% }

% \end{algorithm}

% \begin{algorithm}[h]
% \caption{HeightDistribution}
% \label{alg:coloredHD}
% \Class{$\mathrm{HeightDistribution(\Lambda_o)}$} {

%     \Def{$N, a[], b[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%     \uIf{$N=0$}{
%     $a[1] \gets \Lambda_k$\;
%     $b[1] \gets \Lambda_k$\;
%     $N \gets N+1$\;
%     }
%     \uElseIf{$\Lambda_k < 0$} {
%     \mybox{green}{41.5mm}{
%     \mybox{red}{40mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[i] \gets a[i]\frac{\Lambda_k}{\Lambda_k-b[i]} $\;
%         }
%         }
%         $a[N+1] \gets 0$\;
%         \mybox{red}{40mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[N+1] \gets a[N+1]-a[i] $\;
%         }
%         }
%         $b[N+1] \gets \Lambda_k$\;
%         $N \gets N+1$\;
%     }
%     }
%     \Else{
%     \mybox{yellow}{33.5mm}{
%     \mybox{red}{32mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[i] \gets a[i]\frac{\Lambda_k}{\Lambda_k+b[i]} $\;
%         }
%         }
%         $a[N+1] \gets 0$\;
%         $b[N+1] \gets -\Lambda_k$\;}
%     }
% }
%     \Fn{$\mathrm{getP_{exit}}()$}{
%     \mybox{cyan}{28.5mm}{
%          $s \gets 0$\;
%     \mybox{red}{27mm}{
%         \For{$i \gets 1 ... N$}{
%             $s \gets s + \frac{a[i]}{\Lambda_o+b[i]}$\;
%         }
%         }
%         \KwRet{ s }\;
%         }
    
%     }
% }

% \end{algorithm}

==> sec_implementation.tex <==


\subsection{Efficient BRDF evaluation and sampling}
\label{sec:impl}

\revise{In this section, we show the implementation details of the two key components for a BRDF: evaluation and sample.}

\revise{\paragraph{Evaluation.}
We provide two estimators for BRDF evaluation: a unidirectional estimator using path tracing and a bidirectional estimator using bidirectional path tracing. We provide the details for the unidirectional estimator only, and the bidirectional version is the same as Wang et al.~\shortcite{wang2021positionfree}, except for the segment term.}

\revise{Starting from the incoming ray direction $\bd_0$, we sample the visible normal distribution function to get a new direction and perform the next event estimation by connecting with the outgoing direction $\bd_k$. \revises{The path sampling termination is controlled by the Russian roulette~\cite{Arvo:1990}}. To compute $S_k$ efficiently, we use dynamic programming, as shown in Alg. 1 ( supplementary). }
%\begin{equation}
%\rho (\omega_i,\omega_o)\approx \sum_{i=2}^{i=k+1}\frac{f(\bar{x}_{i})}{\mathrm{pdf}(\bar{x}_{i}) }
%\end{equation}
%Here, we use Russian roulette ~\cite{Arvo:1990} to ensure unbiasedness.}



%我们首先采样出一条既定的路径，随后采用 NEE 计算每个bounce 的贡献，在计算每个 $S_k$ 时我们同样采样DP求解，又因各个bounce之间的路径并不独立，我们在bounce之间复用了DP的中间变量，最终时间复杂度和sample一致，具体细节在伪代码中。我们使用和\cite{wang2021positionfree}一致的 rr 方法，由当前 weight 的最大值决定停止概率。}
%\added{too simple, this is implementation detail. do we use rr?} 

\SetKwProg{Class}{class}{}{end}
\SetKwProg{Fn}{function}{}{end}
\SetKw{Def}{def}
\DontPrintSemicolon

\newcommand{\mycommfont}[1]{\small\texttt{\textcolor[HTML]{4D8F33}{#1}}}
\SetCommentSty{mycommfont}

% \begin{algorithm} 
% \caption{SegmentTerm\_eval}
% \added{\ttfamily include the comments; 算法写的不规范; where is RR?}

% \Class(\tcp*[h]{Initialize $\Lambda_o$}){$\mathrm{SegmentTerm\_eval}(\Lambda_o)$} {

%     $N \gets 0$ \;
%     $m \gets 1$ \;
%     \Def{$e[], g[], l[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%        \eIf{$\Lambda_k < 0$} {
%         $N \gets N+1$\;
%         $l[N] \gets |\Lambda_k|$\;
%         $e[N] \gets \frac{1}{\Lambda_o+|\Lambda_k|}$\;
%         $g[N] \gets 0$\;
%         $m \gets m \cdot e[N]$\Comment{cache the results when sampled rays are only downwards}
%         }{
        
%             \eIf{$m = 0$}
%             {
%                $g[N] \gets \frac{g[N]}{\Lambda_k + l[N]}$\;
%         }(\tcp*[h]{Initialize g}){
%                $g[N] \gets \frac{1}{\Lambda_k + l[N]}$\;
%                $m \gets 0$\;
%             }

%             \For{$i \gets N-1 ... 1$}{
%                 $g[i] \gets \frac{g[i] + g[i + 1]}{\Lambda_k + l[i]}$\;
%             }
%         }
%     }

%     \Fn{$\mathrm{getS_k}()$}{

%         \If(\tcp*[h]{Return results if cached}){$m \ne 0$}{
%         \KwRet{ m }\;
%         }
%          $s \gets 0$\;
%         \For{$i \gets N ... 1$}{
%             $s \gets e[i] \cdot (s + g[i])$\;
%         }
%         \KwRet{ s }\;
    
%     }
% }

% \end{algorithm}

% \begin{algorithm}
% \caption{Eval} 
% \label{alg:eval}
% \Fn{$\mathrm{eval}(\omega_i,\omega_o)$}{
% % \BlankLine
% $\mathrm{SegmentTerm\_eval} \  s(\Lambda(\omega_o))$\Comment{ initializing }
% $f \gets 0$\Comment{result}
% $k \gets 0$ \Comment{bounce}
% $w \gets 1$\Comment{weight}
% $\bd_0 \gets -\omega_i$\;
% \While{$\mathrm{true}$}{
%     $s.\mathrm{addBounce}(\Lambda(\bd_{k}))$\;
%     $S_k \gets s.\mathrm{getS_k}()$\;
%     $k \gets k + 1$\;
%     \If{$k >= rrDepth$}{
%     $q \gets \mathrm{clamp}(S_k,0.3,0.95)$\;
%         \If{$\mathrm{rand}()>q$}{
%         break;
%         }
%     $S_k \gets {S_k \over q}$\;
%     }
%     $f \gets f + w \cdot v(\bd_{k},\omega_o)\cdot S_k $\;
%     \If{$k \ge maxBounce$}{
%         break;
%     }
    
%     ($\bd_{k+1}$,$p_k$) $ \gets $ sample($ \bd_{k} $)\;
%     $w \gets {w \cdot v(\bd_{k},\bd_{k+1}) \over p_k}$\;

% }
%         \KwRet{ f }\;
% }

% \end{algorithm}

\revise{\paragraph{Sample.}
At each bounce, we sample the VNDF to get the outgoing direction and \revise{then compute the masking function ($G_1$ function) of the sampled ray to decide whether to exit the microgeometry}. Otherwise, we treat the sampled direction as the incoming direction and continue sampling until the ray leaves the surface. After getting such a light path, we compute the path contribution by evaluating the light path divided by the PDF \revises{of the sampled path.}}

% \added{in sample, how to decide leave the surface. use the probability for the entire path, or using the masking funciton for the last vertex.}

% \revise{Note that the exit probability can be conditioned on the sampled path, rather than the latest sampled ray. However, the former slightly improves the quality of the rendered image but introduces an extra time overhead. Therefore, we choose the simple way. }
%\revise{我们使用最后一个方向的masking function 决定出射概率，因为我们发现使用整条path来决定出射概率反而更加低效(sample函数大约增加35\%的时间，反应到实际场景上大约增加3\%的渲染时间，但对MSE的影响整体小于1\%).}

% \begin{algorithm}
% \caption{Sample}\label{alg:sample}
% \KwResult{weight $w$ and direction $\bd_k$}
% \BlankLine
% $p \gets 1$  \Comment{pdf}
% $k \gets 0$  \Comment{bounce}
% $w \gets 1$  \Comment{weight}
% $\bd_0 \gets -\omega_i$\;
% \While{$\mathrm{true}$}{
%    ($\bd_k$,$p_k$,$w_k$) $ \gets $ sample($ \bd_{k-1} $)\;
%    $w \gets w \cdot w_k$\;
%    $p \gets p \cdot p_k$\;
%     \If{$\bd_k.z > 0$}{
%     $G_1 \gets \frac{1}{|\Lambda(\bd_k)|}$\;
%         \eIf{$\mathrm{rand()}<G_1$}
%         {
%             $p \gets p \cdot G_1$\;
%             break;
%         }{
%             $p \gets p \cdot (1-G_1)$\;
%         }
%     }
% $k \gets k+1$\;
%     \If{$k \ge maxBounce$}{
%         break;
%     }
% }
%    $w \gets w \cdot S_k(\bd_0,...,\bd_k)$\;
%    $w \gets {w \over p}$\;
% \end{algorithm}


% \myfigure{pdfCurve}{pdfcurve.pdf}{\revise{Comparison between our improved PDF, the previous solution (single bounce + Lambertian term) by Heitz et al.~\shortcite{heitz2016} and the ground truth using the multiple-bounce BRDF reflectance. Our PDF matches the ground-truth PDF at all roughness, while the other solution~\cite{heitz2016} only fits well at high roughness.}}


 \revise{Our key insight is that although an anisotropic \revises{medium} has no analytical multiple-bounce formulation, it can be estimated by an isotropic multiple-bounce formulation derived by Hapke~\shortcite{hapke1981}:}
 \revise{\begin{equation}
\begin{aligned}
f_{\mathrm{mul}}(\omega_i,\omega_o) & = \frac{a}{4\pi}\frac{H\left(\left\vert \omega_g \cdot \omega_i \right \vert\right)H\left(\left\vert \omega_g \cdot \omega_o \right \vert\right)-1}{\left\vert \omega_g \cdot \omega_i \right \vert+\left\vert \omega_g \cdot \omega_o \right \vert},
 \\ H(\mu) & = \frac{1+2\mu}{1+2\sqrt{1-a}\mu},
\end{aligned}
\end{equation}
where $a$ is the \revises{albedo of the medium}.}

\revise{We construct such an isotropic \revises{medium} from the \revises{microfacet}, by setting the \revises{albedo of the medium} as $a = \frac{\alpha_x+\alpha_y}{2}$. Note that this mapping is empirical, due to the observation that the \revises{albedo of the medium} dominates the scattering distribution for an isotropic \revises{medium} and the roughness dominates the scattering distribution for the microfacet model.
Our final PDF includes the single bounce term and the estimated multiple bounce term:
\begin{equation}
\begin{aligned}
f_{\mathrm{PDF}}(\omega_i,\omega_o) & = \frac{D_{\omega_i} \left(\omega_h \right)}{4 \left\vert \omega_h \cdot \omega_i \right \vert}+f_{\mathrm{mul}}(\omega_i,\omega_o).
\end{aligned}
\end{equation}}

\revise{Our PDF matches the ground truth better than the previous estimation combining the single bounce and the Lambertian term, as shown in Figure~\ref{fig:pdfCurve} for both low-roughness and high-roughness materials. Note that our PDF is less accurate for anisotropic BRDFs than for isotropic \revises{medium}, since our mapping function averages the roughness for anisotropic BRDFs. \revises{Our PDF still shows better matching with the ground truth than the single bounce + the Lambertian term approximation, \revises{as shown in Figure 1 (supplementary). Note that an approximated PDF for multiple importance sampling does not introduce bias.}} }



 

%\added{from\cite{hapke1981}: Since the single-scattering term can be evaluated exactly for an arbitrary phase function and the multiply scattered term is relatively insensitive to phase function, a first-order expression for nonisotropic scatterers can be obtained by using the exact expression for singly scattered radiance but retaining the isotropic solution for multiply scattered radiance.}

%\added{\cite{hapke1981} 中对于仅cos的arbitrary phase function有以上的观察，我们拓展了这个观察，认为即使在微表面这种跟方向相关的相位函数，其多重散射也同样可以被 isotropic 的多重散射近似。isotropic 的多重散射在 \cite{amb1943} 中被解析的解出，\cite{hapke1981}对其中的积分部分进行了近似，我们同样也使用这个近似。}
 
 % 我们遵循\cite{hapke1981}中的一个观察，即任意相位函数的半无限体积反射的多重散射部分都可以用各向同性的多重散射近似 （is good to better than 15\%） 
% \revise{因此我们用 albedo  $a = \frac{\alpha_x+\alpha_y}{2}$ 的各向同性半无限体积反射的多重散射部分来替代以往的单一cos项，albedo随粗糙度改变使低粗糙度下也能有较好的表现 （以往没有，导致低粗糙度下glossy的时候 cos仍然占大部分，增大噪声）。所以最终的PDF为：}

%\begin{equation}
%\begin{aligned}
%f_{\mathrm{PDF}}(\omega_i,\omega_o) & = \frac{D_{\omega_i} \left(\omega_h \right)}{4 \left\vert \omega_h \cdot \omega_i \right \vert}+\frac{a}{4\pi}\frac{H\left(\left\vert \omega_g \cdot \omega_i \right \vert\right)H\left(\left\vert \omega_g \cdot \omega_o \right \vert\right)-1}{\left\vert \omega_g \cdot \omega_i \right \vert+\left\vert \omega_g \cdot \omega_o \right \vert}
% \\ H(\mu) & = \frac{1+2\mu}{1+2\sqrt{1-a}\mu}.
%\end{aligned}
%\end{equation}

% Both Heitz et al.~\shortcite{heitz2016} and Wang et al.~\shortcite{wang2021positionfree} used a combination of a single bounce model and a Lambertian term. We use the same strategy. Note that this PDF is used in MIS and it does not have to be accurate.

%We improve this strategy by \added{}. Our PDF is defined as:
%\begin{equation}
% \mathrm{PDF} = \frac{D_{\omega_i} \left(\omega_h \right)}{4 \left\vert \omega_h \cdot \omega_i \right \vert}+\frac{\left\vert \omega_g \cdot \omega_o \right \vert}{\pi}\sqrt{\frac{(\alpha _x\omega_i.x)^2+(\alpha _y\omega_i.y)^2}{1-\omega_i.z^2}}  .
%\end{equation}


==> sup_sec_aniso.tex <==
\section{More results}
As shown in Figure~\ref{fig:anisocurve}, our PDF is less accurate for anisotropic BRDFs than for isotropic media, since our mapping function averages the roughness for anisotropic BRDFs. Even though, our PDF is still better than the single bounce + the Lambertian term approximation.
\myfigure{anisocurve}{pdfcurve_aniso.pdf}{Comparison between our improved PDF, the previous solution (single bounce + the Lambertian term) by Heitz et al.~\shortcite{heitz2016} and the ground truth using the multiple-bounce BRDF reflectance.}

==> sup_sec_compare.tex <==


% \definecolor{main}{HTML}{5989cf}    % setting main color to be used
% \definecolor{sub}{HTML}{cde4ff}     % setting sub color to be used
\subsection{Implementation comparison between our model and Bitterli and d'Eon}

% \begin{algorithm}[t]
% \caption{SegmentTerm}
% \label{alg:coloredST}
% \Class{$\mathrm{SegmentTerm}(\Lambda_o)$} {

%     $N \gets 0$ \;
%     $m \gets 1$ \;
%     \Def{$e[], g[], l[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%        \eIf{$\Lambda_k < 0$} {
%       \mybox{green}{24mm}{
%        % \begin{mybox}[width=30mm]
%        $N \gets N+1$\;
%         % \end{mybox}
%         $l[N] \gets |\Lambda_k|$\;
%         $e[N] \gets \frac{1}{\Lambda_o+|\Lambda_k|}$\;
%         $g[N] \gets 0$\;
%         $m \gets m \cdot e[N]$\;
%         }
%         }{
        
%     \mybox{yellow}{33.5mm}{
%             \eIf{$m = 0$}
%             {
%                $g[N] \gets \frac{g[N]}{\Lambda_k + l[N]}$\;
%         }{
%                $g[N] \gets \frac{1}{\Lambda_k + l[N]}$\;
%                $m \gets 0$\;
%             }
% \mybox{red}{32mm}{
%             \For{$i \gets N-1 ... 1$}{
%                 $g[i] \gets \frac{g[i] + g[i + 1]}{\Lambda_k + l[i]}$\;
%             }}
%             }
%         }
%     }

%     \Fn{$\mathrm{getS_k}()$}{
%     \mybox{cyan}{33.5mm}{
%         \If{$m \ne 0$}{
%         \KwRet{ m }\;
%         }
%          $s \gets 0$\;
         
% \mybox{red}{32mm}{
%         \For{$i \gets N ... 1$}{
%             $s \gets e[i] \cdot (s + g[i])$\;
%         }}
%         \KwRet{ s }\;
%     }
%     }
% }

% \end{algorithm}

% \begin{algorithm}[b]
% \caption{HeightDistribution}
% \label{alg:coloredHD}
% \Class{$\mathrm{HeightDistribution(\Lambda_o)}$} {

%     \Def{$N, a[], b[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%     \uIf{$N=0$}{
%     $a[1] \gets \Lambda_k$\;
%     $b[1] \gets \Lambda_k$\;
%     $N \gets N+1$\;
%     }
%     \uElseIf{$\Lambda_k < 0$} {
%     \mybox{green}{41.5mm}{
%     \mybox{red}{40mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[i] \gets a[i]\frac{\Lambda_k}{\Lambda_k-b[i]} $\;
%         }
%         }
%         $a[N+1] \gets 0$\;
%         \mybox{red}{40mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[N+1] \gets a[N+1]-a[i] $\;
%         }
%         }
%         $b[N+1] \gets \Lambda_k$\;
%         $N \gets N+1$\;
%     }
%     }
%     \Else{
%     \mybox{yellow}{33.5mm}{
%     \mybox{red}{32mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[i] \gets a[i]\frac{\Lambda_k}{\Lambda_k+b[i]} $\;
%         }
%         }
%         $a[N+1] \gets 0$\;
%         $b[N+1] \gets -\Lambda_k$\;}
%     }
% }
%     \Fn{$\mathrm{getP_{exit}}()$}{
%     \mybox{cyan}{28.5mm}{
%          $s \gets 0$\;
%     \mybox{red}{27mm}{
%         \For{$i \gets 1 ... N$}{
%             $s \gets s + \frac{a[i]}{\Lambda_o+b[i]}$\;
%         }
%         }
%         \KwRet{ s }\;
%         }
    
%     }
% }

% \end{algorithm}

% 我们用相同颜色标记了我们和bitterli的算法的主要部分，我们可以看到，在绿色部分中我们没有使用for循环，而bitterli有2次for循环，而在蓝色部分中，我们只有部分情况会有for循环，而bitterli那边始终都会有for循环。

In this section, we compare the implementation details between our segment term and the $p_\mathrm{exit}$ by Bitterli and d'Eon~\shortcite{BitterliAndd'Eon:2022}. We have highlighted the main parts of our algorithm in Alg. \ref{alg:coloredST} and their algorithm in Alg. \ref{alg:coloredHD}. 

The different formulations of the two algorithms lead to different performances. In the end, our method has less time cost when rendered with an equal sample rate.

%For the pseudo-code marked in green, we do not use a  for loop, while Bitterli's algorithm has two for loops. In the blue section, we only have a for loop in certain cases, whereas Bitterli's algorithm always has a for loop.



==> sup_sec_energy.tex <==
\allowdisplaybreaks
\section{BLUE-NOISE TRANSMITTANCE IS  ENERGY CONSERVING}
\label{sec:enervy-conservation}

% We show a simple proof to demonstrate that blue-noise transmittance is energy conserving. We consider a scene filled with a homogeneous participating medium characterized by its extinction coefficient $\sigma\left(s\right)$ and albedo $\alpha$, with the derived scattering coefficient $\sigma_s\left(s\right)=\alpha \sigma\left(s\right)$. We consider a pencil beam of light starting at $x$ traveling in direction $\omega$ that intersects a surface at point $x_z$ . The radiance emitted at the beam origin is $L_0\left(x,\omega\right)$, and the radiance received by points on the beam decreases with distance as a result of extinction by the medium. The emitted radiance must then be distributed between two terms: the amount of light that scatters in the medium, and the remaining fraction that reaches the surface. Assuming a unit albedo, the sum of both terms must equal $L_0\left(x,\omega\right)$—otherwise, energy is either lost or gained along the way. This results in the following constraint:
To demonstrate that blue-noise transmittance conserves energy, we present a straightforward proof. Consider a scene illuminated by a homogeneous participating medium characterized by its extinction coefficient $\sigma\left(s\right)$ and albedo 
$\alpha$, where the scattering coefficient is given by 
$\sigma_s\left(s\right)=\alpha \sigma\left(s\right)$. Suppose a pencil beam of light originating from point 
$x$ travels in direction 
$\omega$ and intersects a surface at point 
$x_z$. The initial radiance of the beam is denoted as 
$L_0\left(x,\omega\right)$. As the light propagates through the medium, the radiance received at points along the beam diminishes due to extinction. Given this setup, the initial radiance must be accounted for by two components: the portion of light that scatters within the medium and the remainder that reaches the surface. With an albedo of one, the sum of these two components must equal the initial radiance 
$L_0\left(x,\omega\right)$. This leads to the following constraint:
\begin{equation}
   L_0(\mathbf{x}, \omega) = L_0(\mathbf{x}, \omega) \text{Tr}(z) + \int_0^z L_0(\mathbf{x}, \omega) \text{Tr}(s) \sigma(s) \, ds,
\end{equation}
The above equation can be simplified by dividing out $L_0\left(x,\omega\right)$:
\begin{equation}
\label{eq:energy_constraint}
1 = \text{Tr}(z) + \int_0^z \text{Tr}(s) \sigma(s) \, ds.
\end{equation}
According to the definition provided in \cite{d_Eon_2018}, we have:
\begin{equation}
\label{eq:blue_definition}
\begin{aligned}
\text{Tr}(z) &= 1-\int_0^z p(s) \,ds, \\
\text{Tr}(s)\sigma(s) &= p(s).
\end{aligned}
\end{equation}
Substituting Eqn.~\ref{eq:blue_definition} into Eqn.~\ref{eq:energy_constraint} yields:
\begin{equation}
1 = 1-\int_0^z p(s)\,ds + \int_0^z p(s) \, ds.
\end{equation}


==> sup_sec_implementation.tex <==

\section{Implementation details}
\label{sec:impl}

In this section, we provide the pseudo-code for our models (both BRDF evaluation and sample) and show the explicit implementation difference between Bitterli and d'Eon~\shortcite{BitterliAndd'Eon:2022} and our model.

\subsection{Implementation details of our model}

% \SetKwProg{Class}{class}{}{end}
% \SetKwProg{Fn}{function}{}{end}
% \SetKw{Def}{def}
% \DontPrintSemicolon

% \newcommand{\mycommfont}[1]{\small\texttt{\textcolor[HTML]{4D8F33}{#1}}}
% \SetCommentSty{mycommfont}

\paragraph{Evaluation}
We provide the pseudo-code of our BRDF evaluation with the unidirectional estimator in Alg.~\ref{alg:eval} and further show the detailed implementation of our segment term using dynamic programming in Alg.~\ref{alg:SegmentTerm}.


\begin{algorithm}[h]
\caption{HeightDistribution (Bitterli and d'Eon)}
\label{alg:coloredHD}
\Class{$\mathrm{HeightDistribution(\Lambda_o)}$} {

    \Def{$N, a[], b[]$} \;

    \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
    \uIf{$N=0$}{
    $a[1] \gets \Lambda_k$\;
    $b[1] \gets \Lambda_k$\;
    $N \gets N+1$\;
    }
    \uElseIf{$\Lambda_k < 0$} {
    \mybox{green}{41.5mm}{
    \mybox{red}{40mm}{
        \For{$i \gets 1 ... N$}{
            $a[i] \gets a[i]\frac{\Lambda_k}{\Lambda_k-b[i]} $\;
        }
        }
        $a[N+1] \gets 0$\;
        \mybox{red}{40mm}{
        \For{$i \gets 1 ... N$}{
            $a[N+1] \gets a[N+1]-a[i] $\;
        }
        }
        $b[N+1] \gets \Lambda_k$\;
        $N \gets N+1$\;
    }
    }
    \Else{
    \mybox{yellow}{33.5mm}{
    \mybox{red}{32mm}{
        \For{$i \gets 1 ... N$}{
            $a[i] \gets a[i]\frac{\Lambda_k}{\Lambda_k+b[i]} $\;
        }
        }
        $a[N+1] \gets 0$\;
        $b[N+1] \gets -\Lambda_k$\;}
    }
}
    \Fn{$\mathrm{getP_{exit}}()$}{
    \mybox{cyan}{28.5mm}{
         $s \gets 0$\;
    \mybox{red}{27mm}{
        \For{$i \gets 1 ... N$}{
            $s \gets s + \frac{a[i]}{\Lambda_o+b[i]}$\;
        }
        }
        \KwRet{ s }\;
        }
    
    }
}

\end{algorithm}

\paragraph{Sample}

We show the multiple-bounce BRDF sample in Alg. \ref{alg:sample}. At each bounce, we sample the VNDF to get the outgoing direction and then compute the masking function ($G_1$ function) of the sampled ray to decide whether to exit the microgeometry. Otherwise, we treat the sampled direction as the incoming direction and continue sampling until the ray leaves the surface. After getting such a light path, we compute the path contribution by evaluating the light path divided by the PDF. Using the masking function of the last sampled ray as the exit probability enables satisfying results with less time cost, while using the entire sampled path to compute the exit probability introduces a large time overhead.

\paragraph{BDPT}

The bidirectional estimator is the same as Wang et al.~\shortcite{wang2021positionfree}, except for the segment term. We did not provide the results of Bitterli and d'Eon \shortcite{BitterliAndd'Eon:2022} (BDPT), since we can not get the correct results after implementing their pseudo-code. We also find that their algorithm does not provide an expected result (single-bounce microfacet BRDF, even set the path length as 2).





==> sup_sec_mixture.tex <==
\allowdisplaybreaks
\section{MIXTURE OF MEDIUM}
\label{sec:mixture}
\paragraph{mixture of medium}
Considering that a medium is a mixture of $n$ different media~\cite{Jarabo_Aliaga_Gutierrez_2018}, and each medium has properties: extinction coefficients $\sigma_t^i$, single-scattering albedo $\alpha^i$, phase function $f_r^i$ and weight $w_i$ ($\sum_{i=1}^n w_i = 1$). We compute the extinction coefficient of mixed medium as:
\begin{equation}
   \sigma_t^{mix}(x,t) = \sum_{i=1}^n w_i\sigma_t^i(x,t),
\end{equation}
where the weight $w_i$ represent the probability of having a scatterer of type $i$. For the phase function and albedo, we have:
\begin{equation}
   \alpha^{mix}(x,t) = \sum_{i=1}^n \frac{w_i \sigma_t^i(x,t)}{\sum_{j=1}^n w_j \sigma_t^j(x,t)}\alpha^i(x,t), 
\end{equation}
\begin{equation}
   f_r^{mix}(x,\omega_i,\omega_o,t) = \sum_{i=1}^n \frac{w_i \sigma_t^i(x,t)\alpha^i(x,t)}{\sum_{j=1}^n w_j \sigma_t^j(x,t)\alpha^j(x,t)}f_r^i(x,\omega_i,\omega_o,t),
\end{equation}
Transmittance $T^{mix}(t)$ and free flight probability density function (PDF) $p^{mix}(t)$ are as follows:
\begin{equation}
\label{eq:T_mix}
\begin{aligned}
    T^{mix}(t) &= e^{-\int_0^z \sigma_t^{mix}(t)dt} \\
    &=\prod_{i=1}^n e^{-\int_0^z w_i \sigma_t^i(t) dt} \\
    &=\prod_{i=1}^n (T^i(t))^{w_i}
\end{aligned}
\end{equation}

\begin{equation}
\label{eq:p_mix}
\begin{aligned}
    p^{mix}(t) &= \frac{-dT^{mix}(t)}{dt}
\end{aligned}
\end{equation}

\paragraph{overlapping of medium} Instead of mixing the medium, consider that a medium is a overlapping of $n$ different media. Each medium has properties: extinction coefficients $\sigma_t^i$, single-scattering albedo $\alpha^i$, phase function $f_r^i$ and density $\rho_i$. We assume that the media are independent of each other. The RTE of this overlapped medium is as follows: 
\begin{equation}
    \begin{aligned}
(\omega \cdot \nabla) L(x, \omega)
&=-\sum_{i=1}^n \rho_i \sigma_{t}^i(x, t) L(x, \omega)  \\
&+\sum_{i=1}^n  \rho_i \sigma_{s}^i(x, t) \int_{\Omega} f_{r}^i\left(x, \omega^{\prime} \cdot \omega, t \right) L\left(x, \omega^{\prime}\right) \mathrm{d} \omega^{\prime}.
\label{eq:rte_overlap}
\end{aligned}
\end{equation}

For simplicity, here we consider the homogeneous case. Integrating both sides of the differential RTE~(\ref{eq:rte_overlap}) along the direction $\omega$ yields the integral form:
\begin{equation}
    \begin{aligned}
    L(x, \omega)=\int_0^\infty T^o(t) \sigma_s^o(t) \int_{\Omega} f_r^o(\omega^{\prime},\omega)L(x+\omega t, \omega^{\prime})\mathrm{d}\omega^{\prime} \mathrm{d}t, \\
\end{aligned}
\end{equation}
where the overlapped transmittance $T^o(t)$, scattering coefficient $\sigma_s^o(t)$ and phase function $f_r^o(\omega_i,\omega_o)$ are given as:
\begin{equation}
\label{eq:T_o}
    \begin{aligned}
    T^{o}(t) &= e^{-\int_0^z \sigma_t^o(t) dt} \\
    \sigma_t^o(t) &= \sum_{i=1}^n \rho_i \sigma_t^{i}(t)
    \end{aligned}
\end{equation}

\begin{equation}
\label{eq:sigmas_o}
    \begin{aligned}
    \sigma_s^{o}(t) &= \sum_{i=1}^n \rho_i \alpha_i(t) \sigma_t^i(t),
    \end{aligned}
\end{equation}

\begin{equation}
\label{eq:fr_o}
   f_r^{o}(\omega_i,\omega_o) = \sum_{i=1}^n \frac{\rho_i \sigma_t^i(t)\alpha^i(t)}{\sum_{j=1}^n \rho_j \sigma_t^j(t)\alpha^j(t)}f_r^i(\omega_i,\omega_o),
\end{equation}
Eqns.~(\ref{eq:T_o}), (\ref{eq:sigmas_o}), and (\ref{eq:fr_o}) have the same form as the formula for the mixed medium, except that the sum of the medium densities $\sum_{i=0}^n\rho_i$ does not need to equal 1.

\paragraph{two traditional medium}
We assume that the saturated medium and the liquid medium are both traditional homogeneous exponential mediums. The extinction coefficient $\sigma_t$, the albedo $\alpha$, and the phase function $f_r$ are independent of $x$ and $t$. We have
\begin{equation}
\label{eq:trad_sigma}
   \sigma_t^{mix} = w_1\sigma_t^{1}+w_2\sigma_t^{2}, 
\end{equation}
\begin{equation}
   \alpha^{mix} = w_1\alpha^{1}+w_2\alpha^{2},
\end{equation}
\begin{equation}
   f_r^{mix}(\omega_i,\omega_o) = \sum_{i=1}^2 \frac{w_i \sigma_t^i\alpha^i}{\sum_{j=1}^2 w_j \sigma_t^j\alpha^j}f_r^i(\omega_i,\omega_o),
\end{equation}
By substituting Eqn.~(\ref{eq:trad_sigma}) into Eqn.~(\ref{eq:T_mix}) and Eqn.~(\ref{eq:p_mix}), we obtain
\begin{equation}
\begin{aligned}
   T_{mix}(t)&=e^{-\sigma_t^{mix}t}, \\
   p_{mix}(t)&=\sigma_t^{mix}e^{-\sigma_t^{mix}t},
\end{aligned}
\end{equation}

\added{In this case, we can use an exponential medium to represent the mixture of mediums. The formulation is simple but we can not integrate porosity into our model.}


\paragraph{blue-noise medium and exponential medium}
We assume that the saturated medium is a blue-noise medium and the liquid medium is an exponential medium. The extinction coefficient $\sigma_t$, the albedo $\alpha$, and the phase function $f_r$ are independent of $x$. We have
\begin{equation}
\label{eq:blue_trad_T}
\begin{aligned}
    T_u^1(t) &=
    \begin{cases}
    1 - \frac{t}{\ell} & 0 \leq t < \hat{t} \\
    \frac{(\ell - \hat{t})e^{-\frac{t - \hat{t}}{\ell-\hat{t}}}}{\ell} & t \geq \hat{t}
    \end{cases} \\
    T_c^1(t) &= 
    \begin{cases}
    1 & 0 \leq t < \hat{t} \\
    e^{-\frac{t - \hat{t}}{\ell - \hat{t}}} & t \geq \hat{t}
    \end{cases} \\
    T^2(t) &= e^{-\sigma_2 t}
\end{aligned}
\end{equation}

By substituting Eqn.~(\ref{eq:blue_trad_T}) into Eqn.~(\ref{eq:T_mix}) and Eqn.~(\ref{eq:p_mix}), we obtain

\begin{equation}
\begin{aligned}
    T_u^{mix}(t) &=
    \begin{cases}
    (1 - \frac{t}{\ell})^{w_1}e^{-w_2 \sigma_2 t} & 0 \leq t < \hat{t} \\
    \left(\frac{(\ell - \hat{t})e^{-\frac{t - \hat{t}}{\ell-\hat{t}}}}{\ell}\right)^{w_1} e^{-w_2 \sigma_2 t} & t \geq \hat{t}
    \end{cases} \\
    T_c^{mix}(t) &= 
    \begin{cases}
    e^{-w_2 \sigma_2 t} & 0 \leq t < \hat{t} \\
    e^{-\left(w_1\frac{t - \hat{t}}{\ell - \hat{t}}+w_2 \sigma_2 t\right)} & t \geq \hat{t}
    \end{cases} \\
\end{aligned}
\end{equation}

\added{In this case, the analytical single scattering is complicated and not reciprocal, but we can integrate porosity into our model.}


\paragraph{Ours}
We assume that the saturated medium is a blue-noise medium and the liquid medium is a specially defined medium. The extinction coefficient $\sigma_t$, the albedo $\alpha$, and the phase function $f_r$ are independent of $x$. We have
\begin{equation}
\label{eq:our_T}
\begin{aligned}
    T_u^1(t) &=
    \begin{cases}
    1 - \frac{t}{\ell} & 0 \leq t < \hat{t} \\
    \frac{(\ell - \hat{t})e^{-\frac{t - \hat{t}}{\ell-\hat{t}}}}{\ell} & t \geq \hat{t}
    \end{cases} \\
    T_c^1(t) &= 
    \begin{cases}
    1 & 0 \leq t < \hat{t} \\
    e^{-\frac{t - \hat{t}}{\ell - \hat{t}}} & t \geq \hat{t}
    \end{cases} \\
    T^2(t) &= 
    \begin{cases}
    1 & 0 \leq t < \hat{t} \\
    e^{-(t - \hat{t})\sigma_2} & t \geq \hat{t}
    \end{cases} \\
\end{aligned}
\end{equation}

By substituting Eqn.~(\ref{eq:our_T}) into Eqn.~(\ref{eq:T_mix}) and Eqn.~(\ref{eq:p_mix}), we obtain ours model.

\added{In this case, the analytical single scattering is cleaner, and we can integrate porosity into our model. However, it is still not reciprocal.}
 







==> sup_sec_single.tex <==
\allowdisplaybreaks
\section{ANALYTICAL SINGLE SCATTERING}
\label{sec:single-scattering}

\paragraph{reflection}
The single scattering BRDF within a medium with thickness $z$ is given by Eqn.~\ref{eq:singleBRDF} (for $cos\omega_i<cos\omega_o$). Since our BSDF is reciprocal, when $cos\omega_i>cos\omega_o$, we need to swap the values of $cos\omega_i$ and $cos\omega_o$ before computation.
% \begin{figure*}[htbp]
% \centering
% \begin{equation}
% \label{eq:singleBRDF}
% f_r\left(\omega_i,\omega_o,z\right)=
% % \frac{\alpha f_p}{\cos\omega_i\cos\omega_o\ell}
% \begin{cases}
% \frac{\alpha f_p \left(1 - e^{-\frac{\left(\cos\omega_i + \cos\omega_o\right) \left(1 + \ell  S  \sigma_t^l\right) z}{\cos\omega_i \cos\omega_o \ell}}\right)}{\left(\cos\omega_i+\cos\omega_o\right)\left(1 + \ell S \sigma_t^l\right)} 
% & \hat{t} = 0 \\
% \frac{\alpha f_p}{cos\omega_o \ell \left(cos\omega_i+cos\omega_o\right)\left(1+\left(\ell-\hat{t}\right)S\omega_t^l\right)} \\
% \left(cos\omega_i\left(\ell+e^{\frac{\left(cos\omega_i-cos\omega_o\right)\hat{t}\left(1+\left(\ell-\hat{t}\right)S\sigma_t^l\right)}{cos\omega_i\left(\ell-\hat{t}\right)}}\left(-\ell+\hat{t}\right)+\ell\hat{t}S\sigma_t^l-\hat{t}^2S\sigma_t^l\right) \right.\\
% \left.
% +cos\omega_o\left(\ell+e^{\frac{\left(1+\left(\ell-\hat{t}\right)S\sigma_t^l\right)\left(2cos\omega_i cos\omega_o\hat{t}-\left(cos\omega_i+cos\omega_o\right)z\right)}{cos\omega_i cos\omega_o\left(\ell-\hat{t}\right)}}\left(-\ell+\hat{t}\right)+\ell\hat{t}S\sigma_t^l-\hat{t}^2S\sigma_t^l\right)\right)
% & \cos\omega_o \, \hat{t} < z \, \\
% \frac{\alpha f_p \left(\ell+e^{\frac{\left(1+\left(\ell-\hat{t}\right)S\sigma_t^l\right)\left(cos\omega_i\hat{t}-z\right)}{cos\omega_i\left(\ell-\hat{t}\right)}}\left(-\ell+\hat{t}\right)+\ell\hat{t}S\sigma_t^l-\hat{t}^2S\sigma_t^l\right)}{cos\omega_o \ell \left(1+\left(\ell-\hat{t}\right)S\sigma_t^l\right)} 
% & \cos\omega_i \, \hat{t} < z \, \&\& \, \cos\omega_o \, \hat{t} \geq z \, \\
% \frac{z \alpha f_p}{cos\omega_i cos\omega_o \ell}
% & \text{otherwise}
% \end{cases}
% \end{equation}
% \end{figure*}

% \newcommand{\abs}[1]{\lvert #1 \rvert}

% \paragraph{transmission}
% Similarly, the single scattering BTDF within a medium with thickness $z$ is given by Eqn.~\ref{eq:singleBTDF} (for $\abs{cos\omega_i}<\abs{cos\omega_o}$).
% \begin{figure*}[htbp]
% \centering
% \begin{equation}
% \label{eq:singleBTDF}
% \begin{aligned}
% f_t\left(\omega_i,\omega_o,z\right) &=
% \frac{\alpha f_p \left(X_1+X_2+X_3+X_4
% \right)}{\abs{cos\omega_i} \abs{cos\omega_o} \ell} \\
% X_1 &= 
% \begin{cases}
%  \frac{\abs{cos\omega_o} e^{\frac{((l-\hat{t}) S \sigma_t^l+1) (\abs{cos\omega_o} \hat{t}-z)}{\abs{cos\omega_o}
%    (l-\hat{t})}} \left(-1+e^{\frac{\abs{cos\omega_i} \hat{t} \left(S
%    \sigma_t^l+\frac{1}{l-\hat{t}}\right)}{\abs{cos\omega_o}}}\right) (l-\hat{t})}{(l-\hat{t}) S
%    \sigma_t^l+1} &  z>(\abs{cos\omega_i}+\abs{cos\omega_o}) \hat{t} \\
%  -\frac{\abs{cos\omega_o} \left(-1+e^ {\frac{((l-\hat{t}) S \sigma_t^l+1) (\abs{cos\omega_o}
%    \hat{t}-z)}{\abs{cos\omega_o} (l-\hat{t})}}\right) (l-\hat{t})}{(l-\hat{t}) S \sigma_t^l+1} &
%     \abs{cos\omega_o} \hat{t}<z \leq (\abs{cos\omega_i}+\abs{cos\omega_o}) \hat{t} \\
% \end{cases} \\
% X_2 &= 
% \begin{cases}
%  -\frac{\abs{cos\omega_i} e^ {\frac{((\ell-\hat{t}) S \sigma_t^l+1) ((\abs{cos\omega_i}+\abs{cos\omega_o})
%    \hat{t}-z)}{\abs{cos\omega_i} (\ell-\hat{t})}} \left(-1+e^{\frac{\abs{cos\omega_o} \hat{t} ((\hat{t}-\ell) S
%    \sigma_t^l-1)}{\abs{cos\omega_i} (\ell-\hat{t})}}\right) (\ell-\hat{t})}{(\ell-\hat{t}) S \sigma_t^l+1} 
%    & z\geq (\abs{cos\omega_i}+\abs{cos\omega_o}) \hat{t} \\
%  \frac{\abs{cos\omega_i} e^{-\frac{\ell S \sigma_t^l z+z}{\abs{cos\omega_i} \ell-\abs{cos\omega_i} \hat{t}}} \left(-e^
%    {\frac{\hat{t} ((\ell-\hat{t}) S \sigma_t^l \abs{cos\omega_i}+\abs{cos\omega_i}+S \sigma_t^l
%    z)}{\abs{cos\omega_i} (\ell-\hat{t})}}+e^{\frac{\ell S \sigma_t^l z+z}{\abs{cos\omega_i} \ell-\abs{cos\omega_i}
%    \hat{t}}}\right) (\ell-\hat{t})}{(\ell-\hat{t}) S \sigma_t^l+1} 
%    & \abs{cos\omega_i} \hat{t}<z<(\abs{cos\omega_i}+\abs{cos\omega_o}) \hat{t} \\
% \end{cases}\\
% X_3 &= 
% \begin{cases}
%  \abs{cos\omega_i} \hat{t} & \abs{cos\omega_i} \hat{t}<z\leq \abs{cos\omega_o} \hat{t} \\
%  z & z\leq \abs{cos\omega_i} \hat{t} \\
%  (\abs{cos\omega_i}+\abs{cos\omega_o}) \hat{t}-z & \abs{cos\omega_o} \hat{t}<z<(\abs{cos\omega_i}+\abs{cos\omega_o}) \hat{t} \\
% \end{cases}\\
% X_4 &= 
% \begin{cases}
%  \frac{\abs{cos\omega_i} \abs{cos\omega_o} e^ {\frac{((\ell-\hat{t}) S \sigma_t^l+1) (2 \abs{cos\omega_o}
%    \hat{t}-z)}{\abs{cos\omega_o} (\ell-\hat{t})}} \left(-e^ {\frac{(\abs{cos\omega_i}-\abs{cos\omega_o}) \hat{t}
%    ((\ell-\hat{t}) S \sigma_t^l+1)}{\abs{cos\omega_o} (\ell-\hat{t})}}+e^ {\frac{(\abs{cos\omega_i}-\abs{cos\omega_o})
%    ((\ell-\hat{t}) S \sigma_t^l+1) (z-\abs{cos\omega_o} \hat{t})}{\abs{cos\omega_i} \abs{cos\omega_o}
%    (\ell-\hat{t})}}\right) (\ell-\hat{t})}{(\abs{cos\omega_i}-\abs{cos\omega_o}) ((\ell-\hat{t}) S \sigma_t^l+1)} 
%    & z>(\abs{cos\omega_i}+\abs{cos\omega_o}) \hat{t} \\
%  \frac{\abs{cos\omega_i} \abs{cos\omega_o} e^{-\frac{\ell S \sigma_t^l z+z}{\abs{cos\omega_o} \ell}}
%    \left(-1+e^{\frac{(\abs{cos\omega_i}-\abs{cos\omega_o}) (\ell S \sigma_t^l+1) z}{\abs{cos\omega_i} \abs{cos\omega_o} \ell}}\right)
%    \ell}{(\abs{cos\omega_i}-\abs{cos\omega_o}) (\ell S \sigma_t^l+1)} & \hat{t} = 0 \\
% \end{cases}\\
% \end{aligned}
% \end{equation}
% \end{figure*}

==> sup_sec_slab.tex <==
\section{Formulation for medium slab}
\label{supsec:slab}
% 对medium slab的推导与论文中对微表面的推导基本一致，考虑厚度为$T$的medium slab，从下方减去一层厚度为$\Delta\tau$的薄层，并加在slab的顶面上，设反射和透射的多重散射相位函数分别为$\rho_r$和$\rho_t$，列出发生改变几种情况即可得到最终的表达式。要注意的是透射还会额外的考虑一个Delta transmission。
The derivation for the medium slab is similar to the derivation for microfacet in the paper. Considering a medium slab with a thickness of $T$, we subtract a thin layer with a thickness of $\Delta\tau$ from the bottom and add it to the top surface of the slab. Let $\rho_r$ and $\rho_t$ represent the multiple scattering phase functions for reflection and transmission, respectively. By considering various cases where changes occur, we can obtain the final expressions. It is important to note that transmission also includes delta transmission.
\subsection{Reflection}
% \textbf{:}
\begin{equation}
\begin{aligned}
&\rho _r\left(\omega_{i}, \omega_{o}\right) = \frac{1}{\Lambda\left(-\omega_{i}\right)+\Lambda\left(\omega_{o}\right)}\bigg(v\left(\omega_{i}, \omega_{o}\right)+\\
&\int_{\Omega^+}\Big(\rho _r\left(\omega_{i}, \omega\right) v\left(\omega, \omega_{o}\right)+v\left(\omega_{i},-\omega\right) \rho _r\left(-\omega, \omega_{o}\right)\Big) \mathrm{d} \omega \\
&+\int_{\Omega^+} \int_{\Omega^+}\Big(\rho _r\left(\omega_{i}, \omega_{1}\right) v\left(\omega_{1},-\omega_{2}\right)\rho _r\left(-\omega_{2}, \omega_{o}\right)-\\
&\rho _t\left(\omega_{i},-\omega_{1}\right) v\left(-\omega_{1}, \omega_{2}\right) \rho _t\left(-\omega_{2}, -\omega_{o}\right)\Big) \mathrm{d} \omega_{1} \mathrm{~d} \omega_{2}\bigg).
\end{aligned}
\end{equation}
% 透射：
\subsection{Transmission}
% \textbf{Transmission:}

\begin{equation}
\begin{aligned}
&\rho _t\left(\omega_{i}, \omega_{o}\right) = \delta\left(\left\|\omega_{i}-\omega_{o}\right\|\right) e^{-T \Lambda\left(-\omega_{i}\right)}+\frac{1}{\Lambda\left(-\omega_{i}\right)+\Lambda\left(\omega_{o}\right)}\\
&\bigg(\int_{\Omega^+}\Big(v\left(\omega_{i},-\omega\right) \rho_t\left(-\omega, \omega_{o}\right)-\rho_t\left(\omega_{i},-\omega\right) v\left(-\omega, \omega_{o}\right)\Big) \mathrm{d} \omega \\
&+\int_{\Omega^+} \int_{\Omega^+}\Big(\rho_r\left(\omega_{i}, \omega_{1}\right) v\left(\omega_{1},-\omega_{2}\right)\rho_t\left(-\omega_{2}, \omega_{o}\right)-\\
&\rho_t\left(\omega_{i},-\omega_{1}\right) v\left(-\omega_{1}, \omega_{2}\right) \rho_r\left(-\omega_{2}, -\omega_{o}\right)\Big) \mathrm{d} \omega_{1} \mathrm{~d} \omega_{2}\bigg).
\end{aligned}
\end{equation}

==> temp_method_refraction.tex <==
\subsection{Multi-bounce formulation for the refractive microfacet model}
\label{sec:refraction}

%对于折射，来说，事情变得复杂了起来，我们需要用4组带深度的积分方程来描述其过程：

We also use the variance principle for the refractive surfaces. Different from the reflective surface, there are four combinations considering the inside / outside of the surface and the reflection or refraction interaction. We use $\rho_r^{o}$ and $\rho_r^{i}$ to represent reflection at the outside / inside of the surface respectively. We use $\rho_t^{o}$ to represent the refraction from the outside to the inside of the surface, and $\rho_t^{i}$ for the vice versa.

For each of these four cases, we formulate the changes of the radiance via the invariance principle. The question is how to derive the formulation in the refraction case. In the reflective surface, we model the microfacet model as a homogeneous media and add a layer on top of the media; then we derive the multiple scattering formulation using the invariance principle. However, for the refractive surface, the derivation is not as simple as the reflection case. 

在反射情况下，只用了线性主部，但是在折射中没有办法只用线性主部。为什么？或者说为什么在折射情况下需要在下面去掉一个layer， 而在reflection情况下不需要去掉这个layer。以及去掉这个layer的含义到底是什么。
另外，是如何model的，仍然是medium么还是说用height field。用medium又应该如何解释呢？

So, for the refractive case, we model the media as \added{xxx}. Then add a layer on top of the media and reduce a layer at the bottom. Then we will show how these two layers change the four cases ($\rho_r^o,\rho_r^{i},\rho_t^o,\rho_t^{i}$). We only provide the full derivation of the $\rho_r^{o}$ in the main paper and \added{leave the others in the supplementary.} 

\myfigure{refractionCases}{refractionCases.png}{\added{The first case is missing.} Six cases of $\rho_r^{o}$ due to the adding of the thin layer on a refractive microgeometry. \added{Redraw later.} }

We first consider both the incoming light and the outgoing light locates outside the surface with a reflection interaction. Adding a layer on the top of the medium and reducing a layer at the bottom results in six cases, including the four cases in the reflection. The other two cases are:
\begin{itemize}
    \item one refractive interactions along the incoming ray $\omega_i$, represented as $TT^*$,
    \item one refractive interactions along the outgoing ray $\omega_o$, represented as $T^*T$.
\end{itemize}
Therefore, we have: $R^*, R, RR^*,R^*R, TT^*$, and $T^*T$. Do we only have these six cases? As we talked earlier in the reflection case, we only consider at most one scattering event in the adding layer, since more scattering events are quantities of a higher order of smallness relative to $\Delta \tau$. Besides these six cases, do we have other cases with at most one scattering event in the adding layer? Note that, the current case is about $\rho_r^{o}$, so the entire light transport should be a reflection and only even count of $T$ or $T^*$ is required. We also have $R^*RR^*$, $T^*RT^*$, \added{$R^*TT^*$ or $T^*TR^*$}. However, these four cases do not exist, since the reflection event at the outside of the surface can only happens at the upper hemisphere and vise versa. 

The next question is how to compute the contribution of the two new cases ($T^*T$ and $TT^*$) with refraction. \added{Here, we define K}.

Given the six cases of radiance change for $\rho_r^{o}$, we get the following equation to keep energy conservation: 
% \begin{equation}
% \begin{aligned}
% &\rho^o_r\left(\omega_{i}, \omega_{o}\right)= \frac{1}{\Lambda\left(-\omega_{i}\right)+\Lambda\left(\omega_{o}\right)+1}\bigg(v^o_r\left(\omega_{i}, \omega_{o}\right)+\\
% &\int _{\Omega^+}\Big( v^o_r\left(\omega_{i}, -\omega\right)\rho^o_r \left(-\omega, \omega_{o}\right)+\rho^o_r\left(\omega_{i}, \omega\right) v^o_r\left(\omega, \omega_{o}\right)\Big) \mathrm{d}\omega \bigg)+\\
% &\int^\infty_{0}\bigg(\int _{\Omega^+}\Big(e^{-\tau|\Lambda\left(\omega_{i}\right)|}v^o_t\left(\omega_{i}, \omega\right)\rho^i_t\left(\left | \ln\left ( 1-e^{-\tau} \right )   \right | ,\infty,-\omega, -\omega_o\right)\\
% &+\rho^o_t\left(0,\tau,\omega_{i}, -\omega\right)v^i_t\left(\omega, -\omega_o\right)e^{-\left | \ln\left ( 1-e^{-\tau} \right )   \right |\Lambda\left(\omega_{o}\right)}\Big)\mathrm{d}\omega\bigg)\mathrm{d}\tau\\
% \end{aligned}
% \end{equation}
\begin{equation}
\begin{aligned}
&(\rho^o_r\left(\omega_{i}, \omega_{o}\right)-K_{TvT\rho}-K_{T\rho Tv})(|\Lambda\left(\omega_{i}\right)|+\Lambda\left(\omega_{o}\right))= \bigg(v^o_r\left(\omega_{i}, \omega_{o}\right)+\\
&\int _{\Omega^+}\Big( v^o_r\left(\omega_{i}, -\omega\right)\rho^o_r \left(-\omega, \omega_{o}\right)+\rho^o_r\left(\omega_{i}, \omega\right) v^o_r\left(\omega, \omega_{o}\right)\Big) \mathrm{d}\omega \bigg)\\
\end{aligned}
\end{equation}

%\begin{equation}
%\begin{aligned}
%&(\rho^o_t\left(\omega_{i}, \omega_{o}\right)-K_{Tv}-K_{TvR\rho}-K_{R\rho Tv})(|\Lambda\left(\omega_{i}\right)|-\Lambda\left(-\omega_{o}\right))=\\
%&\int _{\Omega^+}\Big( v^o_r\left(\omega_{i}, -\omega\right)\rho^o_t \left(-\omega, \omega_{o}\right)-\rho^o_t\left(\omega_{i}, -\omega\right) v^i_r\left(-\omega, \omega_{o}\right)\Big) \mathrm{d}\omega\\
%\end{aligned}
%\end{equation}

Similarly to the $\rho^o_r$, we also derive the formulation for other three cases, where the details are shown in the supplementary.

% \begin{equation}
% \begin{aligned}
% &\rho^i_r\left(\omega_{i}, \omega_{o}\right)= \frac{1}{\Lambda\left(-\omega_{i}\right)+\Lambda\left(\omega_{o}\right)+1}\bigg(v^i_r\left(\omega_{i}, \omega_{o}\right)+\\
% &\int _{\Omega^+}\Big( v^i_r\left(\omega_{i}, -\omega\right)\rho^i_r \left(-\omega, \omega_{o}\right)+\rho^i_r\left(\omega_{i}, \omega\right) v^i_r\left(\omega, \omega_{o}\right)\Big) \mathrm{d}\omega \bigg)+\\
% &\int^\infty_{0}\bigg(\int _{\Omega^+}\Big(e^{-\tau|\Lambda\left(\omega_{i}\right)|}v^i_t\left(\omega_{i}, \omega\right)\rho^o_t\left(\left | \ln\left ( 1-e^{-\tau} \right )   \right | ,\infty,-\omega, -\omega_o\right)\\
% &+\rho^i_t\left(0,\tau,\omega_{i}, -\omega\right)v^o_t\left(\omega, -\omega_o\right)e^{-\left | \ln\left ( 1-e^{-\tau} \right )   \right |\Lambda\left(\omega_{o}\right)}\Big)\mathrm{d}\omega \bigg)\mathrm{d}\tau\\
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% &\rho^o_t\left(\tau_i,\tau_o,\omega_{i}, \omega_{o}\right)=\\
% &\int^{\max(\tau_i,\tau_o)}_{\min(\tau_i,\tau_o)}\bigg(e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}v^o_t\left(\omega_{i}, \omega_{o}\right)e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}  \right |\right|\Lambda\left(-\omega_{o}\right)} \\
% &+\int _{\Omega^+}\Big(\rho^o_t\left (\tau_i,\tau, \omega_i,-\omega\right )v^i_r(\omega,-\omega_o)e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\\
% &+e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}v^o_r(\omega_i,-\omega)\rho^o_t\left (\tau,\tau_o,-\omega, \omega_o \right ) \Big) \mathrm{d}\omega \bigg)\mathrm{d}\tau\\
% &+\int^\infty_{\tau_i} e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\mathrm{d}\tau\\
% &\times \int _{\Omega^+} v^o_t\left(\omega_{i}, \omega\right)\rho^i_r \left(-\omega, -\omega_{o}\right)\mathrm{d}\omega\\
% &+\int^{\tau_o}_0 e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\mathrm{d}\tau\\
% &\times \int _{\Omega^+} \rho^o_r\left(\omega_{i}, \omega\right) v^o_t\left(\omega, \omega_{o}\right)\mathrm{d}\omega\\
% &\rho^o_t\left(\omega_{i}, \omega_{o}\right)=\rho^o_t\left(0,\infty,\omega_{i}, \omega_{o}\right)\\
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% &\rho^i_t\left(\tau_i,\tau_o,\omega_{i}, \omega_{o}\right)=\\
% &\int^{\max(\tau_i,\tau_o)}_{\min(\tau_i,\tau_o)}\bigg(e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}v^i_t\left(\omega_{i}, \omega_{o}\right)e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}  \right |\right|\Lambda\left(-\omega_{o}\right)} \\
% &+\int _{\Omega^+}\Big(\rho^i_t\left (\tau_i,\tau, \omega_i,-\omega\right )v^o_r(\omega,-\omega_o)e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\\
% &+e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}v^i_r(\omega_i,-\omega)\rho^i_t\left (\tau,\tau_o,-\omega, \omega_o \right ) \Big) \mathrm{d}\omega \bigg)\mathrm{d}\tau\\
% &+\int^\infty_{\tau_i} e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\mathrm{d}\tau\\
% &\times \int _{\Omega^+} v^i_t\left(\omega_{i}, \omega\right)\rho^o_r \left(-\omega, -\omega_{o}\right)\mathrm{d}\omega\\
% &+\int^{\tau_o}_0 e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\mathrm{d}\tau\\
% &\times \int _{\Omega^+} \rho^i_r\left(\omega_{i}, \omega\right) v^i_t\left(\omega, \omega_{o}\right)\mathrm{d}\omega\\
% &\rho^i_t\left(\omega_{i}, \omega_{o}\right)=\rho^i_t\left(0,\infty,\omega_{i}, \omega_{o}\right)\\
% \end{aligned}
% \end{equation}

In the reflection case, the shadowing-masking function for a light path can be easily obtained with the equation from the invariance principle. However, in the refraction case, we can not get the shadowing-masking function for a light path obviously, given the above four equations. We introduce the hypergeometric functions to solve these equations.

The hypergeometric functions are introduced by Gauss~\shortcite{gauss1812} and later extended to generalized hypergeometric functions by Pochhammer~\shortcite{pochhammer1870}, which are defined by infinite series:

%对此，我们并不能给出一个任意阶折射pathG的递归式。但我们仍然可以将其计算出来。

%我们首先需要引入一些数学工具。

%Gauss~\shortcite{gauss1812} 引入了超几何函数 ${_{2}F_{1}}$, Pochhammer~\shortcite{pochhammer1870} 将其推广为了广义超几何函数 ${_{p}F_{q}}$. 这些函数由无穷级数定义:
\begin{equation}
     \begin{aligned}
{_{p}F_{q}}\left(a_1,a_2,\cdots,a_p;b_1,b_2,\cdots,b_q,z\right)=\sum_{k=0}^{\infty}\frac{{\Tiny\displaystyle\prod_{i=1}^{p}} \frac{\Gamma \left ( a_i+k\right)}{\Gamma\left(a_i\right)}}{{\Tiny\displaystyle\prod_{j=1}^{q}}\frac{\Gamma \left ( b_j +k\right ) }{\Gamma \left ( b_j\right )}}\frac{z^k}{k!},
     \end{aligned}
    \label{eq:hypergeometric}
\end{equation}
 where $\Gamma$ is the Gamma function, and $(x-1)!$ is the analytic continuation. \added{We also need to define the other notations.}
 %$\Gamma$ 是伽马函数, 是 $(x-1)!$ 的解析延拓.

As we know the shadowing-masking function of a single bounce for the refractive surface is given by Pinel et al.~\shortcite{Pinel:05} using the Beta function:

%单次折射的pathG $S_{\mathrm{T}}$ 在\cite{Pinel:05}中已经给出, 其中用到了Beta函数:

\begin{equation}
     \begin{aligned}
    \mathrm{B}(a, b)=\int_{0}^{1} t^{a-1}(1-t)^{b-1} \mathrm{~d}t.
     \end{aligned}
    \label{eq:beta}
\end{equation}

Note that the Beta function and the Gamma function has the following relationship:
%这些函数有如下关系:
\begin{equation}
     \begin{aligned}
    \mathrm{B}(a, b)=\frac{\Gamma(a)\Gamma(b)}{\Gamma(a+b)}=\frac{1}{a}{_{2}F_{1}}(a,1-b;1+a,1).
     \end{aligned}
\end{equation}

However, we find that the Beta function can not solve the shadowing-masking function for more bounces. Thus, we propose a novel function, called \emph{generalized Beta functions}, which are defined as:
%当我们试图解决反射问题时，我们发现现有的数学工具已经无法满足我们的需要，我们得定义一些新函数，我们称为 \emph{generalized beta functions}:
\begin{equation}
     \begin{aligned}
 &\mathrm{B}^k(a_1,a_2,\cdots,a_k;b_1,b_2,\cdots,b_k)=\\ &\int_{\displaystyle [0,1]\times \prod_{m=1}^{k-1}[0,u_m ] }\prod_{n=1}^{k} u_n^{a_n-1}(1-u_n)^{b_n-1}\mathrm{~d}\mu\left(\overline{u}\right),
     \end{aligned}
    \label{eq:generalizedbeta}
\end{equation}
where $\mathrm{B}^1(a_1;b_1)=\mathrm{B}(a_1,b_1)$.

%这个函数有许多好的性质，例如对称性：
Note that this function is symmetric:
\begin{equation}
     \begin{aligned}
 &\mathrm{B}^k(a_1,a_2,\cdots,a_k;b_1,b_2,\cdots,b_k)=\\
 &\mathrm{B}^k(b_k,b_{k-1},\cdots,b_1;a_k,a_{k-1},\cdots,a_1)
     \end{aligned}
\end{equation}
\added{Note that we can not prove this symmetric property, but we check the numerical values.}

With the generalized Beta function, we finally derive the shadowing-masking function for a path with refraction. 
%We can derive some equations for at least three bounces. For more bounces, 
%定义了这些之后，我们就可以表示出带有折射的pathG。

%以下是包含折射的2次散射的所有pathG：
The shadowing-masking function for a path with refraction-reflection is: 

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TR}}\left(\mathbf{d}_{0}, \mathbf{d}_{1}, \mathbf{d}_{2}\right)=\\
&\begin{cases}
\frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{1}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|)-\mathrm{B}(|\Lambda\left(\mathbf{d}_{2}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{|\Lambda\left(\mathbf{d}_{2}\right)|-|\Lambda\left(\mathbf{d}_{1}\right)|}, \text { if } \mathbf{d}_{1} . z<0 \\
\frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{2}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{|\Lambda\left(\mathbf{d}_{2}\right)|+\Lambda\left(\mathbf{d}_{1}\right)}, \text { if } \mathbf{d}_{1} . z>0
\end{cases}
     \end{aligned}
\end{equation}

The reflection-refraction case is symmetric to the above equation, thus we show it in the supplementary. Then we show the equation for the refraction-refraction case:

% \begin{equation}
%      \begin{aligned}
% &S_{\mathrm{RT}}\left(\mathbf{d}_{0}, \mathbf{d}_{1}, \mathbf{d}_{2}\right)=\\
% &\begin{cases}
% \frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{1}\right)|,|\Lambda\left(\mathbf{d}_{2}\right)|)-\mathrm{B}(|\Lambda\left(\mathbf{d}_{2}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{|\Lambda\left(\mathbf{d}_{0}\right)|-|\Lambda\left(\mathbf{d}_{1}\right)|}, \text { if } \mathbf{d}_{1} . z<0 \\
% \frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{2}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{|\Lambda\left(\mathbf{d}_{0}\right)|+\Lambda\left(\mathbf{d}_{1}\right)}, \text { if } \mathbf{d}_{1} . z>0
% \end{cases}
%      \end{aligned}
% \end{equation}

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TT}}\left(\mathbf{d}_{0}, \mathbf{d}_{1}, \mathbf{d}_{2}\right)=\\
&\begin{cases}
\mathrm{B}^2(|\Lambda\left(\mathbf{d}_{0}\right)|,\Lambda\left(\mathbf{d}_{2}\right)+1;-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1), \text { if } \mathbf{d}_{1} . z<0 \\
\mathrm{B}^2(\Lambda\left(\mathbf{d}_{2}\right)+1,|\Lambda\left(\mathbf{d}_{0}\right)|;\Lambda\left(\mathbf{d}_{1}\right)+1,-\Lambda\left(\mathbf{d}_{1}\right)), \text { if } \mathbf{d}_{1} . z>0
\end{cases}
     \end{aligned}
\end{equation}

%3次：

For three bounces, we show the TRR (RRT), RTR, TTR (RTT), TRT and TTT.

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TRR}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\frac{\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{2}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|}-\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{3}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|}}{\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|\right)},\\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{2}\right)\right|+\Lambda\left(\mathbf{d}_{1}\right)}-\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{3}\right)\right|+\Lambda\left(\mathbf{d}_{1}\right)}}{\left|\Lambda\left(\mathbf{d}_{3}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{3}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{(|\Lambda\left(\mathbf{d}_{3}\right)|+\Lambda\left(\mathbf{d}_{2}\right))(|\Lambda\left(\mathbf{d}_{3}\right)|+\Lambda\left(\mathbf{d}_{1}\right))}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
&S_{\mathrm{RTR}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\frac{\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{2}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|}-\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|}}{\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|\right)}, \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left(\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|\right)\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|+\Lambda\left(\mathbf{d}_{2}\right)\right)}, \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0\\
\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|\right)\left(\left|\Lambda\left(\mathbf{d}_{0}\right)\right|+\Lambda\left(\mathbf{d}_{1}\right)\right)}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{3}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{(|\Lambda\left(\mathbf{d}_{3}\right)|+\Lambda\left(\mathbf{d}_{2}\right))(|\Lambda\left(\mathbf{d}_{0}\right)|+\Lambda\left(\mathbf{d}_{1}\right))}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
\end{cases}
     \end{aligned}
\end{equation}

% \begin{equation}
%      \begin{aligned}
% &S_{\mathrm{RRT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
% &\begin{cases}
% \frac{\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{1}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|}-\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|}}{\left(\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|\right)}, \\
% \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
% \frac{\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{1}\right)\right|+\Lambda\left(\mathbf{d}_{2}\right)}-\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{0}\right)\right|+\Lambda\left(\mathbf{d}_{2}\right)}}{\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|}, \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0\\
% \frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{3}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{(|\Lambda\left(\mathbf{d}_{0}\right)|+\Lambda\left(\mathbf{d}_{2}\right))(|\Lambda\left(\mathbf{d}_{0}\right)|+\Lambda\left(\mathbf{d}_{1}\right))}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
% \end{cases}
%      \end{aligned}
% \end{equation}

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TTR}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\frac{\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{1}\right)+1,-\Lambda\left(\mathbf{d}_{1}\right);\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\Lambda\left(\mathbf{d}_{3}\right)-\Lambda\left(\mathbf{d}_{2}\right)}, \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{1}{\Lambda\left(\mathbf{d}_{3}\right)-\Lambda\left(\mathbf{d}_{2}\right)}(\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{1}\right)+1,-\Lambda\left(\mathbf{d}_{1}\right);\Lambda\left(\mathbf{d}_{2}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)\\
-\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{1}\right)+1,-\Lambda\left(\mathbf{d}_{1}\right);\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)), \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0\\
\frac{\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)}{\Lambda\left(\mathbf{d}_{3}\right)-\Lambda\left(\mathbf{d}_{2}\right)}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{1}{\Lambda\left(\mathbf{d}_{3}\right)-\Lambda\left(\mathbf{d}_{2}\right)}(\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{2}\right)+1\right)\\
-\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)), \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TRT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\frac{1}{\Lambda\left(\mathbf{d}_{1}\right)-\Lambda\left(\mathbf{d}_{2}\right)}(\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{1}\right)+1,-\Lambda\left(\mathbf{d}_{1}\right);\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)\\
-\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{2}\right)+1,-\Lambda\left(\mathbf{d}_{2}\right);\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)), \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{1}{\Lambda\left(\mathbf{d}_{1}\right)-\Lambda\left(\mathbf{d}_{2}\right)}(\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{2}\right)+1,-\Lambda\left(\mathbf{d}_{2}\right);\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)\\
+\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)), \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{1}{\Lambda\left(\mathbf{d}_{1}\right)-\Lambda\left(\mathbf{d}_{2}\right)}(\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{2}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)\\
-\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)), \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
\end{cases}
     \end{aligned}
\end{equation}

% \begin{equation}
%      \begin{aligned}
% &S_{\mathrm{RTT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
% &\begin{cases}
% \frac{1}{\Lambda\left(\mathbf{d}_{1}\right)+\left|\Lambda\left(\mathbf{d}_{0}\right)\right|}(\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{2}\right)+1,-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{1}\right)\right|\right)\\
% -\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{2}\right)+1,-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)),\\
% \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
% \frac{\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{2}\right)+1,-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\Lambda\left(\mathbf{d}_{1}\right)+\left|\Lambda\left(\mathbf{d}_{0}\right)\right|}, \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0\\
% \frac{1}{\Lambda\left(\mathbf{d}_{1}\right)+\left|\Lambda\left(\mathbf{d}_{0}\right)\right|}(\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{2}\right)+1,\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)\\
% -\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{2}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)), \\
% \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
% \frac{\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{2}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)}{\Lambda\left(\mathbf{d}_{1}\right)+\left|\Lambda\left(\mathbf{d}_{0}\right)\right|}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
% \end{cases}
%      \end{aligned}
% \end{equation}

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TTT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\mathrm{B}^3(|\Lambda(\mathbf{d}_0)|,\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2);-\Lambda(\mathbf{d}_1),\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|), \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
\mathrm{B}(|\Lambda(\mathbf{d}_0)|,-\Lambda(\mathbf{d}_1))\mathrm{B}^2(\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|;\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2))\\
-\mathrm{B}^3(-\Lambda(\mathbf{d}_1),\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|;|\Lambda(\mathbf{d}_0)|,\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2)), \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0\\
\mathrm{B}(|\Lambda(\mathbf{d}_0)|,-\Lambda(\mathbf{d}_1))\mathrm{B}^2(\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2);\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|)\\
-\mathrm{B}^3(|\Lambda(\mathbf{d}_0)|,\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2);-\Lambda(\mathbf{d}_1),\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|), \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
\mathrm{B}^3(-\Lambda(\mathbf{d}_1),\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|;|\Lambda(\mathbf{d}_0)|,\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2)), \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
\end{cases}
     \end{aligned}
\end{equation}

The equation for more bounces can be similarly derived. For a light path with $n$ refractive interactions can be represented with a n-order generalized Beta function.  

The next question is how to solve these generalized Beta function. For the two-order generalized Beta function, we have:
%对于二次的广义beta函数，我们可以得到：

\begin{equation}
\begin{aligned}
&\mathrm{B}^2(a_1,a_2;b_1,b_2)  \\
=& \frac{1}{a_2}\mathrm{B}\left ( a_1+a_2,b_1 \right ) {_{3}F_{2}}\left ( a_2,1-b_2,a_1+a_2;a_2+1,a_1+a_2+b_1,1 \right ). \\
\end{aligned}
\end{equation}

However, for higher orders, the generalized Beta function can not be solved analytically bu the current mathematical tool, and we leave this problem for the future work. 

To summarize, we can provide the formulation of the refractive surface with any bounces, but the current mathematical tool can only solve at most two refractive interactions. Therefore, we use our proposed model for all the reflection case with any bounce, all the two-bounce cases and all the three-bounce cases except TTT. We leave the other cases with the random walk solution, similar to Heitz et al.~\shortcite{heitz2016}.

% \begin{equation}
% \begin{aligned}
% &\mathrm{B}^2(a_1,a_2;b_1,b_2)  \\
% =& \int_{0}^{1} \int_{0}^{\mathcal{U}_1} \mathcal{U}_1^{a_1-1}(1-\mathcal{U}_1)^{b_1-1}\mathcal{U}_2^{a_2-1}(1-\mathcal{U}_2)^{b_2-1}\mathrm{~d}\mathcal{U}_2\mathrm{d}\mathcal{U}_1 \\
% =& \int_{0}^{1} \mathcal{U}_1^{a_1-1}(1-\mathcal{U}_1)^{b_1-1}\mathrm{B}(\mathcal{U}_1 ;a_2,b_2) \mathrm{~d}\mathcal{U}_1 \\
% =&\frac{1}{a_2}\int_{0}^{1} \mathcal{U}_1^{a_1+a_2-1}(1-\mathcal{U}_1)^{b_1-1}{_{2}F_{1}}(a_2,1-b_2;1+a_2,\mathcal{U}_1) \mathrm{~d}\mathcal{U}_1 \\
% =&\frac{1}{a_2}\sum_{k=0}^{\infty}\left ( \frac{\frac{\Gamma \left ( a_2+k\right)}{\Gamma\left(a_2\right)}\frac{\Gamma \left ( 1-b_2+k\right)}{\Gamma\left(1-b_2\right)}}{\frac{\Gamma \left ( a_2+1+k\right ) }{\Gamma \left ( a_2+1\right )}k!}\int_{0}^{1} \mathcal{U}_1^{a_1+a_2+k-1}(1-\mathcal{U}_1)^{b_1-1} \mathrm{~d}\mathcal{U}_1 \right ) \\
% =&\frac{1}{a_2}\sum_{k=0}^{\infty}\left ( \frac{\frac{\Gamma \left ( a_2+k\right)}{\Gamma\left(a_2\right)}\frac{\Gamma \left ( 1-b_2+k\right)}{\Gamma\left(1-b_2\right)}}{\frac{\Gamma \left ( a_2+1+k\right ) }{\Gamma \left ( a_2+1\right )}k!}\frac{\Gamma \left ( a_1+a_2+k\right ) \Gamma \left ( b_1\right )}{\Gamma \left ( a_1+a_2+b_1+k\right )} \right ) \\
% =&\frac{1}{a_2}\sum_{k=0}^{\infty}\left ( \frac{\frac{\Gamma \left ( a_2+k\right)}{\Gamma\left(a_2\right)}\frac{\Gamma \left ( 1-b_2+k\right)}{\Gamma\left(1-b_2\right)}}{\frac{\Gamma \left ( a_2+1+k\right ) }{\Gamma \left ( a_2+1\right )}k!}\frac{\frac{\Gamma \left ( a_1+a_2+k\right )}{\Gamma \left ( a_1+a_2\right )}}{\frac{\Gamma \left ( a_1+a_2+b_1+k\right )}{\Gamma \left ( a_1+a_2+b_1\right )} } \right )\frac{\Gamma \left ( a_1+a_2\right )\Gamma \left ( b_1\right )}{\Gamma \left ( a_1+a_2+b_1\right )}  \\
% =& \frac{1}{a_2}\mathrm{B}\left ( a_1+a_2,b_1 \right ) {_{3}F_{2}}\left ( a_2,1-b_2,a_1+a_2;a_2+1,a_1+a_2+b_1,1 \right ) \\
% \end{aligned}
% \end{equation}

%但可惜的是，三次及以上的广义beta函数并不能被现有的数学工具解析的表示，我们只能把这个问题留给数学界。

%我们可以表明的是，含有n次折射过程的pathG，其中必含有n次的广义beta函数，所以我们目前只能解析的计算所有纯粹反射，带折射的所有2次的情况及除了 TTT 以外的所有3次的情况，对于其他的情况，我们回退到随机游走进行计算。


